Robust Calibration For Improved Weather Prediction Under Distributional Shift

In this paper, we present results on improving out-of-domain weather prediction and uncertainty estimation as part of the \texttt{Shifts Challenge on Robustness and Uncertainty under Real-World Distributional Shift} challenge. We find that by leveraging a mixture of experts in conjunction with an advanced data augmentation technique borrowed from the computer vision domain, in conjunction with robust \textit{post-hoc} calibration of predictive uncertainties, we can potentially achieve more accurate and better-calibrated results with deep neural networks than with boosted tree models for tabular data. We quantify our predictions using several metrics and propose several future lines of inquiry and experimentation to boost performance.

==> data_metrics.tex <==
\section{Dataset}

We employ the use of the Shifts Dataset developed by Yandex Research for the Shifts Challenge. The dataset comprises of pairs of meteorological features and air tempretures 2 metres above ground for a diverse set of latitudes and longitudes. The goal of this dataset is to predict air temperature at 2 meters above ground at a particular latitude/longitude and timestamp, given all available weather station measurements and multiple weather forecast model predictions.

There are two specific set of feature categories that make up this datset: Weather-related features and Meteorological features. Weather related features consist of sun evaluation at the current location, climate values of temperature, pressure and topography. Meteorological parameters are detailed based on pressure and surface level data from the weather prediction models. 

There are five climate types associated with the dataset: Tropical, Dry, Mild Temperate, Snow and Polar. The dataset is split amounts training, development and testing based on the climate associated with features, in order to provide a clear distributional shift in the weather data. The training data consists of features with climate types as Tropical, Dry and Mild Temperature. This data is recorded from 1st September 2018, to 8th April, 2019. The development data has the same climate types as the training data, apart from one distributionally shifted set consisting of features only with the climate type Snow. The evaluation dataset has been shifted based on climate and time. The evaluation dataset consists of features with Snow and Polar climate types, recorded from 14th May,2019 to 8th July,2019.

The split in the training, development and evaluation data show a clear distributional shift, presenting a challenge to develop models robust to these shifts and competent at generalisation to OOD data.

\section{metrics}
We assess the predictive performance of our model using Root Mean Squared Estimation and Mean Absolute Error. For a predicted value {x_{i}} and ground truth {y_{i}}, we calculate the RMSE as:
RMSE = \sqrt{(\frac{1}{n})\sum_{i=1}^{n}(y_{i} - x_{i})^{2}}

We calculate MAE as :
MAE = {(\frac{1}{n})\sum_{i=1}^{n}(y_{i} - x_{i})^{2}}

We assess the uncertainity via error-retention and F1-retention curves. We use R-AUC and F1-AUC as metrics to calculate uncertainty.A good uncertainty measure is able to achieve low R-AUC and high F1-AUC.Additionally, the F1 score at a retention rate of 95\% of the most certain samples is also quoted and is denoted as F1@95\%, which is a single point summary jointly of the uncertainty and robustness. Finally, ROC-AUC is used as a summary statistic for evaluating uncertainty-based out-of-distribution data detection.
